LLM-Based Website Classification for Targeted Web Measurements

Web measurements based on top lists of popular websites are a well-established methodology for assessing the security and privacy landscape of the Internet. However, existing top lists are unlabeled and lack semantic information about the nature of the included websites, forcing researchers to rely on custom techniques to focus on specific website classes of interest. This makes targeted web measurements, e.g., over shopping websites, challenging to carry out. In this paper, we investigate the use of Large Language Models (LLMs) to enable targeted web measurement studies. Building on prior literature, we identify key website classification tasks relevant to web measurements and highlight limitations in state-of-the-art classification approaches. We thus construct more carefully curated datasets to evaluate different LLMs on these tasks using standard performance measures. Our results show that LLMs can achieve strong performance across multiple classification scenarios, but the choice of the model and its configuration play a significant role in both the quality and the efficiency of the classification process. Finally, we use LLMs to emulate the setup of a targeted web measurement by automatically detecting adult websites in a subset of the Tranco list, without any need for custom techniques for dataset construction. Together, our benchmark evaluation and case study show that LLMs can enable high-quality targeted web measurements at scale directly over the Tranco list.

==> measurements-old.tex <==
\section{LLM-Assisted Web Measurements}
\label{sec:measurement}
\SC{Leftover dalla versione precedente, da aggiungere a questa sezione: We ground our investigation on the Tranco list generated on 22 December 2025~\cite{TrancoDec}. When performing web measurements tasks, we visit the landing page of each website from within an academic network, using a lightweight crawler controlled by an LLM via LangChain. The crawler is based on the Chromium browser, operated in headful mode through Playwright. Each website is accessed using a fresh browser instance with a clean profile.}

\revision{In the previous section, we evaluated several LLMs for website classification on our benchmark datasets and found that gpt-oss consistently outperformed the other models. We also conducted a scalability analysis, showing that LLM-based classification can support large-scale measurements, though with a trade-off between accuracy and performance. Building on these results, we propose an LLM-based methodology that leverages the Tranco list and can serve as a foundation for large-scale targeted web measurements. We then evaluate it in a realistic setting by conducting two large-scale targeted web measurements and assessing whether the resulting inferences are reliable and consistent with prior literature.}
%Here, we take an additional step and investigate to what extent gpt-oss can serve as the backbone of web measurement studies. To ground this analysis in a realistic setting, we consider the common practice of conducting measurements over top lists of popular websites like Tranco~\cite{PochatGTKJ19}. Since Tranco is unannotated in nature, measurements that are geared towards specific classes of websites require ad-hoc filtering to only keep the targets of interest. This can be challenging and require carefully crafted heuristics, as we discussed before. In the following sections, we assess how the use of simple ad-hoc heuristics from the literature fares against the use of general automated inferences performed by LLM. \revision{We also evaluate the scalability of using an LLM for building a targeted dataset in the context of our web measurement studies (in Appendix~\ref{app:scalability}).}

\subsection{The Two-Step Filtering Methodology}

%\SC{Qui vogliamo dire che i dataset della letteratura sono stati dimostrati sotto-ottimali. Idealmente nel mondo measurement tutti usano Tranco, ma non possiamo usarlo as is per targeted measurement. C'è un trade-off: accedere tutto e classificare può essere costoso, quindi proponiamo due passate (figura). Nelle prossime sezioni dimostriamo che tale metodologia che combina precisione con performance è robusta perché riproduciamo research inferences esistenti.}

%\SC{Questa sezione è un wall of text e senza la figura è veramente too much. Andrebbe organizzata in maniera opportuna per migliorarne la leggibilità, es. usando paragrafi / itemize esattamente come abbiamo fatto nel resto del paper. Qui è dove c'è il contributo innovativo, deve essere leggibile.}
%\LC{Userei come titolo della sottosezione proprio il nome della metodologia.}
\subsubsection{Motivation.} 
\revision{Web measurements are typically conducted using the Tranco list, which has become the de facto standard in the field and has been adopted by more than 600 academic publications. However, Tranco is unannotated. As a result, measurements targeting specific classes of websites require ad-hoc filtering or heuristic-based dataset construction methods to isolate the domains of interest. As discussed previously, no de facto standard exists for this task, and current state-of-the-art techniques exhibit biases and limitations due to the intrinsic difficulty of accurately classifying websites (Section~\ref{sec:survey}). While we improved upon existing approaches (Section~\ref{sec:benchmark}), our solution still suffers from unavoidable biases and limitations. Moreover, the methodology must often be adapted on a case-by-case basis, requiring different ad-hoc solutions depending on the measurement target.}
\SC{Per la methodology: meglio avere una figura che chiarisca l'idea, facendo anche vedere le alternative. Mi sembra ci siano tre possibilità naturali: classification URL-only + visita ai positivi, classification con access + visita ai positivi, visita a tutti i siti a prescindere. La nostra metodologia fa qualcosa di ancora diverso. Da rifletterci con calma.}

\subsubsection{Methodology.}
\revision{We propose a new methodology that can serve as a general foundation for large-scale targeted web measurements. Starting from the Tranco list, we use an LLM to filter domains and retain only those relevant to the measurement objective, reducing potential bias introduced by ad-hoc heuristics. As shown in the previous section, LLMs achieve high classification accuracy, especially when granted access to website content, making them well-suited for this task. In addition, LLM-based classification improves scalability, since many domains can be classified without visiting the corresponding websites. This is important because website visits substantially increase the runtime of LLM-based inference pipelines. This creates a trade-off: classification without website access is faster but less precise than classification with access enabled. To balance efficiency and accuracy, we propose a two-step filtering strategy that minimizes website visits while maintaining high classification performance:}

\begin{enumerate}
    \item \revision{\emph{Fast Pre-Filtering:}} \revision{We first filter the raw Tranco list using LLM-based classification without website access. This step is much faster than traditional heuristic-based or human-driven approaches, which require visiting every website, as well as LLM classification with website access enabled. It discards most irrelevant domains and retains only a smaller subset of potentially relevant ones.}

    \item \revision{\emph{High-Precision Refinement:}} \revision{We then apply a second filtering step using LLM classification with website access enabled. Although more expensive, it is applied only to the reduced subset and provides the highest classification accuracy, improving the quality and reliability of the final dataset.}
\end{enumerate}

Overall, the proposed methodology is both accurate and scalable, as supported by our previous analyses. It can be applied to any targeted web measurement study while mitigating the biases and limitations of prior state-of-the-art approaches. Based on the execution times measured in Section~\ref{sec:scalability}, we estimate that classifying the Tranco top 100k, a moderately sized list requires on average 3 days and 11 hours with our methodology, assuming that only 10\% of websites pass the first filtering step, in line with the observations reported in the next section. This is faster than traditional approaches, which require visiting every website and take an estimated 7 days and 7 hours on average. 
Moreover, it saves roughly a day compared to LLM classification with live access alone (4 days and 9 hours on average), even though the latter is fast enough to be usable when filtering 100k websites.
The advantage of our methodology becomes evident for larger lists, where live access dominates the overall cost, as stated in Section~\ref{sec:scalability}. Under the same assumptions, classifying the Tranco top 1M takes 34 days and 11 hours on average with our approach, compared to 72 days and 22 hours with traditional methods and 43 days and 23 hours with LLM classification with live access enabled. This represents a substantial improvement, bringing the runtime much closer to the estimated 30 days and 2 hours required by LLM classification without website access, while producing a more reliable dataset thanks to the second filtering step.
\SC{Qui sarebbe molto più evocativo avere un plot che faccia vedere l'andamento stimato per i tempi per i tre approcci naturali e la nostra metodologia. Potremmo poi confrontarlo dopo con dati reali almeno su una scala più piccola (es. 10k, corrispondenti ad un punto dell'asse x).}

%Estimates:
%3 days without website access on average for 100k websites
%4 days and 9 hours with website access on average for 100k websites

%1M without access: 30 days and 2 hours, 722.222 hours
%1M with access: 43 days and 23 hours, 1055,555 hours

%\LC{ Per quanto questa aggiunta non faccia male, ometterei la stima del tempo medio per l'operazione di filtro, dato che ci manca il riscontro ottenuto dall'applicazione della metodologia, come viene indicato da una nota successiva. Dalla sezione precedente emerge già che, in media, la classificazione con o senza website access è più veloce in media del tempo medio di visita di un sito.}

%\subsubsection{Strengths and Limitations.}
\revision{This methodology is well-suited for targeted web measurements because, unlike traditional web measurements, they do not require visiting every website in the Tranco list. Instead, the measurement is only performed on a specific subset of domains matching the target category, which typically represents only a fraction of Tranco. The main limitation of this approach is susceptibility to false negatives, since the first filtering step is less precise than the second, while false positives are largely eliminated in the second step. Nevertheless, we expect false negatives to remain limited, as LLM classification without website access still achieves high macro F1 (Section~\ref{sec:classification-performance}). Moreover, this is acceptable in our setting, since our primary goal is to build accurate and reliable datasets to support subsequent measurements. In the next sections, we validate our methodology by conducting two large-scale targeted web measurements and evaluating whether the resulting research inferences are consistent with those reported in prior work.}

%\SB{Da fare la figura e aggiungerla (che ci sia spazio? forse non serve la figura dato che la metodologia è molto semplice).}
%\LC{Va bene accennare qui alle limitazioni dell'approccio. Teniamo comunque conto che ci potrebbe essere richiesto di proporre un'analisi quantitativa riguardo i benifici di questa strategia: su un sample di Tranco, per i due task di classificazione presi in considerazione qui sotto, riportare i falsi negativi e falsi positivi ottenuti con le due strategie di filtro e poi dalla metodologia con le due passate. Penso sia un punto da revision, in caso.}

\subsection{Dataset Construction}

\revision{To assess whether our methodology can support the construction of reliable and representative datasets for targeted web measurements, we consider two prominent case studies from the literature. In particular, we focus on privacy analyses of governmental~\cite{GotzeMISL22,SamarasingheAMY22,SinganamallaJAK20} and pornographic~\cite{VallinaFGVA19} websites, both of which require ad-hoc dataset construction for the measurement task, a process that is inherently challenging and lacks standardization. We begin by applying our methodology to build two datasets from the Tranco top 1M. Then, we use them to perform the corresponding web measurements and compare the resulting research inferences with those obtained using the independent ad-hoc datasets proposed in prior work~\cite{GotzeMISL22,SinganamallaJAK20,VallinaFGVA19}.}

\revision{We build both datasets using gpt-oss, which achieved the best performance in our evaluation (Section~\ref{sec:classification}). From the Tranco top 1M, we selected the top 50k and bottom 50k domains to obtain an initial pool of 100k websites spanning a wide range of popularity levels. We then apply a first filtering step using gpt-oss, classifying domains as governmental based solely on their URLs. This yielded an intermediate dataset of 5,631 domains. Next, following our two-step approach, we asked gpt-oss to reclassify these domains with live access to the corresponding websites, rather than relying exclusively on URL information. After this refinement step, the final dataset contains 2,475 governmental websites.}

\revision{In parallel, we applied the same procedure to construct a dataset of pornographic websites. Starting from the same pool of 100k domains, we first used gpt-oss to classify websites as pornographic based solely on their URLs, yielding an intermediate set of 8,949 domains. We then reclassified these domains with live access to the corresponding websites, resulting in a dataset of 2,936 pornographic websites. Additional details on the quality of the resulting datasets, as well as a comparison with traditional heuristic-based approaches, are provided in Appendix~\ref{app:measurement_dataset_construction}.}

\SC{Forse le due sezioni dopo si possono proprio togliere. Andrebbero invece confrontate le metodologie possibili a livello di classificazione (falsi positivi, falsi negativi) e tempi di measurement in maniera completa. Anche su Tranco Top 10k se vogliamo accelerare i tempi, ma va fatto per bene.}

%\SB{Forse fa un po' strano qui non riportare il tempo totale impiegato, ma non ce l'abbiamo...}
%\LC{Mi sembra che andiamo fin troppo diretti a parlare di governmental e porn datasets, ma prima non abbiamo mai detto che ci saremmo concentrati su questi due measurements e quindi sulla costruzione di due dataset appositi. Basterebbe solo introdurre questo all'inizio di questa sezione (con una riga/due sulla motivazione, magari ribadendo il fatto che la costruzione dei dataset per questi due measurement è challenging, come fatto nella precedente versione del paper).}
% \subsection{Targeted Web Measurements}
% Web measurements are routinely performed over top lists of popular websites like Tranco~\cite{PochatGTKJ19}. Since Tranco is unannotated in nature, measurements that are geared towards specific classes of websites require ad-hoc filtering to only keep the targets of interest. This can be challenging and require carefully crafted heuristics, as we discussed before. In this section, we experimentally estimate how the use of simple ad-hoc heuristics from the literature fares against the use of general automated inferences performed by LLM.

% In our first experiment we deal with governmental websites, a prominent target of prior work~\cite{GotzeMISL22,SamarasingheAMY22,SinganamallaJAK20}. Starting from the Tranco top 1M, we selected the top 50k and the bottom 50k websites to come up with an initial list of websites of diverse popularity. We then filtered the resulting 100k websites to only keep those hosted under an extensive list of known top-level domains associated with governments~\cite{GotzeMISL22}. This process led to a corpus of XXX websites. We then fed the 100k websites from Tranco to chat-gpt and used it to keep only those that were classified as governmental, leading to a dataset of YYY websites.

%\SC{Vediamo intanto i numeri, ne scopriamo molti di più? Quanto overlappano? Da un punto di vista qualitativo osserviamo qualcosa di interessante? Per esempio la Germania non ha un suffisso gov dedicato, quindi LLM sembra l'unica strada. Ci saranno poi molti paesi piccoli che LLM becca ma non sono coperti da suffissi noti. A me pare un'analisi da riportare. Questo dataset si può poi usare direttamente nella sezione 6.3.}

%We now move to our second experiment on associating websites with the country of their target audience, which is a useful task when measuring compliance with respect to privacy regulations~\cite{...}. Starting from the previously selected 100k websites from Tranco, we assigned a country to them based on their top-level domain as proposed by Ogut et al.~\cite{OgutTMLYCU24}. This allowed us to categorize XXX websites to a set of different countries including China, Germany, India, Indonesia, Italy, Japan, Korea, Netherlands and Turkey. The significant decrease in numbers mostly comes from the presence of many generic top-level domains like .com in the considered slice of Tranco. To mitigate this issue, we tried to perform country attribution based on the signals explored in the construction of the Countries dataset. In particular, we accessed each website with a browser set to English and we assigned it the country $c$ provided that $(i)$ the language of its homepage matches the primary language of $c$ and $(ii)$ the IP address of the host serving the content is in the same continent of $c$. We then used gpt-oss for country association, leading to a set of XXX websites from the different countries.
%\SC{Vediamo intanto i numeri, ne categorizziamo molti di più? Da un punto di vista qualitativo osserviamo qualcosa di interessante? Da vedere.}

%\SC{Altri casi di studio, tipo pornographic websites o simili? Sarebbe utile anche per convincere che le performance non ottimali osservate per Categories in realtà sono meglio di ciò che dicono quei numeri. Farebbe vedere anche la generalità ad altri measurement tasks considerati in letteratura.}
%\SC{Sezione 6 dovrebbe anche discutere le performance, che sono importanti per large-scale measurements. Teniamo traccia di quanto ci ha messo a classificare 100k siti per i vari task.}

% \subsection{Privacy Risks of Single Sign-On}

% \writtenbyLC{We start by exploring the privacy risks of SSO. Dimova et al.~\cite{DimovaGJ23} presented a tool to assess such risks in existing SSO deployments and used it to measure their prevalence in the wild. The tool detects the presence of SSO on websites, identifies the available identity providers, and extracts the \emph{scopes} requested during authentication, i.e., the type and amount of user information a website requests. A scope is considered \emph{minimal} when it includes only the necessary information required for a given identity provider, and a website mitigates privacy risks when it consistently requests minimal scopes. As a part of their study, Dimova et al.~\cite{DimovaGJ23} further reported a breakdown of the websites minimizing privacy risks (in terms of requested scopes) across different website categories. This work is a good example of how website categorization can complement web measurements by uncovering correlations between website categories and privacy/security best practices. For website classification, the study relies on the commercial McAfee SiteAdvisor tool~\cite{mcafee-siteadvisor}, which is freely available for occasional individual use but not intended for large-scale analyses under its terms of service.}\footnote{Dimova et al. likely relied on SiteAdvisor under a large-scale use agreement~\cite{mcafee-siteadvisor}.}

% \writtenbyLC{We replicate the study performed by Dimova et al. about the privacy risks per website category using Gemini, to understand if LLMs can help in drawing similar inferences. In particular, we downloaded the original dataset by Dimova et al. along with its website categories from SiteAdvisor and reassigned the categories using Gemini. For simplicity and readability, our analysis covers just the 10 most popular categories in the dataset, accounting for 2,912 websites from the original study (47\%). Note that the categories assigned by SiteAdvisor are different from those available in the Curlie dataset considered in Section~\ref{sec:classification}, hence our prompt for Gemini was adapted accordingly. Moreover, we instructed Gemini to assign only one label per website. Recall that in Section~\ref{sec:classification-results-categories} we requested two labels from Gemini to compensate for the underlabeling of Curlie, while, in this case, requiring a single label allows us to be coherent with the categorization provided by SiteAdvisor.}

% \writtenbyLC{Figure~\ref{fig:dimova_cat} compares the results of the privacy analysis using the original SiteAdvisor classification and the Gemini classification. As it turns out, the privacy inferences are nearly identical for the two classification tools across the vast majority of the categories. For example, the difference observed in the Forum/Bulletin category amounts to 1.4\%, where websites requesting minimal scope amount to 72.0\% and 70.6\% according to Gemini's and SiteAdvisor's classification, respectively. The largest observed discrepancy between the two categorizations, and arguably the only notable one, is 8.2\% for the Blogs/Wiki category. However, this difference does not significantly affect the overall conclusions of the analysis, because Blogs/Wiki still ranks among the last two categories in terms of the percentage of websites requesting minimal scopes. This result confirms that a commercial website classification service can be effectively replaced by a general-purpose LLM, provided it is properly instructed about the semantics of the target categories.}

% \writtenbyLC{To further assess the consistency of the inferences that can be drawn using LLMs for website categorization, we conduct an additional experiment focusing on the two most popular identity providers in the dataset, i.e., Google and Facebook. Precisely, we compare the percentage of websites requesting minimal scopes across categories for these providers, using both Gemini's and SiteAdvisor's classifications. This way, we can evaluate if the LLM-based categorization leads to similar privacy-related conclusions when the analysis is centered on identity providers rather than on websites alone. The results again confirm that the conclusions derived from both classifications are consistent. Detailed results are reported in Appendix~\ref{sec:sso-idps}.}

% \SB{Magari mostrare in qualche modo che la distribuzione è la stessa perchè i siti sono stati categorizzati allo stesso modo e non perchè le label sono state invertite tra i siti. Cioè non abbiamo ottenuto la stessa distribuzione dove però i siti categorizzati sotto quelle label sono diversi da quelli categorizzati sotto quelle label in dimova. Non saprei come mostrare questa cosa e se abbia senso.}
% \SB{Possiamo contare il numero di volte in cui i siti sono stati categorizzati diversamente tra i due dataset.}
% \SB{Spostare appendice B nel main body? Forse abbiamo spazio...}
% %In particular, the percentage of websites requesting minimal scope is above 85\% for all the considered categories when Facebook, Google and Twitter are the identity providers. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.42]{plots/plot_gemini_categorization_1_bucket_final.png}
%     \caption{Percentage of websites with minimal scope by category, comparing SiteAdvisor and Gemini classification.}
%     \label{fig:dimova_cat}
% \end{figure}=

\subsection{Privacy of Governmental Websites}
\label{sec:gov_privacy_analysis}

%\SB{Ho tolto analysis dai titoli, così non vanno a capo, ma non so se vada bene.}

%In our first study, we focus on governmental websites, a prominent target of prior work~\cite{GotzeMISL22,SamarasingheAMY22,SinganamallaJAK20}, which has, for instance, examined the privacy risks of e-government practices by analyzing the cookies set by these sites. A significant challenge of these studies is the construction of an ad-hoc dataset of governmental websites for the measurement task. This process lacks standardized grounds and prior work relied on seeds of known governmental websites to identify more websites to include in the dataset by means of web crawling. We here explore to what extent the adoption of LLM-filtered versions of the Tranco list may allow performing representative web measurements, leading to similar conclusions to those observed on a carefully constructed, ad-hoc dataset of governmental websites.

%\subsubsection{Dataset Construction}
%\label{sec:gov_privacy_analysis-dataset}
%We begin by constructing our gpt-oss filtered dataset, evaluating its quality, and comparing it with a simple TLD-based heuristic approach. Starting from the Tranco top 1M, we selected the top 50k and the bottom 50k websites to come up with an initial list of websites of diverse popularity. From this set of 100k websites, we first applied a heuristic filter based on an extensive list of top-level domains (TLDs) known to be associated with governmental entities~\cite{GotzeMISL22}. This process yielded a corpus of 821 websites, which we use as a baseline. In parallel, we applied gpt-oss to the same set of 100k domains and selected those classified as governmental based solely on their URLs, resulting in a substantially larger dataset of 5,631 websites. To improve dataset quality and reduce false positives, we introduced a second filtering phase. In this step, we asked gpt-oss to reclassify the previously selected domains, this time allowing live access to the corresponding websites rather than relying exclusively on the URL. After this refinement process, the resulting dataset contains 2,475 websites. 
%\revision{The two-step filtering process required a total of 17 days and 13 hours, comprising 17 days and 6.5 hours for the first phase and 6.5 hours for the second. Further analysis of LLM scalability for large-scale website classification is provided in Appendix~\ref{app:scalability}.}

%To assess the quality of both approaches, we randomly sampled 50 websites from each dataset and manually inspected them. All 50 websites drawn from the TLD-filtered dataset were confirmed to be governmental, confirming the reliability of this heuristic and supporting its use as a baseline for constructing a dataset of governmental websites. For the LLM-based dataset, 46 out of 50 websites (92\%) were correctly identified as governmental, indicating high dataset quality. When comparing the gpt-oss filtered dataset with the baseline, we observe a substantial overlap of 751 websites, corresponding to 91\% of the baseline dataset; 70 domains are unique to the baseline, whereas 1,724 appear exclusively in the gpt-oss filtered dataset. These results suggest that although the LLM misses a small number of domains with specific governmental TLDs, which are likely to be governmental, it successfully detects a large number of governmental websites that do not rely on such TLDs and are therefore missed by the baseline. Consequently, the LLM-based dataset can be considered an improvement over the baseline, substantially extending it while maintaining high accuracy (92\%).

%A representative example illustrating the limitations of TLD-based classification is Germany, which does not use a dedicated governmental top-level domain. In such cases, identifying governmental websites becomes more challenging, as no explicit indicator clearly distinguishes them from other types of entities. Accurate classification therefore requires a more semantically informed analysis, such as that provided by an LLM.
%\SC{Attenzione qui. Lavori esistenti su governmental website hanno coperto anche la Germania senza usare LLM, quindi la conclusione è debole. Andrebbe chiarita meglio la rappresentatività di questo esperimento. Non so se il modo giusto sia presentare la collezione dei .gov come un modo per costruire il dataset, perchè altri paper hanno fatto altri, quindi forse è solo una semplice baseline per fare sanity check rispetto a ciò che hai costruito con gpt-oss. Se lo presentassimo così, si sistemerebbe anche il mio secondo appunto (vedi dopo).}

%\subsubsection{Web Measurement}
%\label{sec:gov_privacy_analysis-dataset-measurement}
%In our first study, we focus on governmental websites, a prominent target of prior work~\cite{GotzeMISL22,SamarasingheAMY22,SinganamallaJAK20}. To assess whether the proposed methodology is effective at building a dataset that is representative and supports meaningful research inferences, we perform a privacy analysis measuring the prevalence of third-party cookies set by known trackers on governmental websites, based on the Disconnect list~\cite{disconnect_tracking_protection}. We then compare these results with two independent, ad-hoc datasets of governmental websites~\cite{GotzeMISL22,SinganamallaJAK20}, applying the same methodology.\footnote{We cannot compare also with the dataset of~\cite{SamarasingheAMY22} because it is not publicly available.} Specifically, we run the tool built by Gotze et al.~\cite{GotzeMISL22} over all three datasets to collect the relevant data, and then process it to evaluate tracker prevalence and popularity. %We focus exclusively on the gpt-oss filtered dataset, as it provides a more comprehensive dataset than the previously presented baseline.
%\SC{Occhio anche qui. Uno potrebbe chiedersi perchè non usi il dataset con i soli .gov che hai costruito prima. Che fine ha fatto quello?}

In our first study, we focus on governmental websites, a prominent target in prior work~\cite{GotzeMISL22,SamarasingheAMY22,SinganamallaJAK20}. To evaluate whether our methodology can construct a representative dataset and support meaningful research inferences, we conduct a privacy analysis measuring the prevalence of third-party cookies set by known trackers on governmental websites, using the Disconnect tracking protection list~\cite{disconnect_tracking_protection}. We then compare our findings against results obtained from two independent, ad-hoc governmental website datasets proposed in the literature~\cite{GotzeMISL22,SinganamallaJAK20}, applying the same analysis methodology.\footnote{We cannot compare with the dataset of~\cite{SamarasingheAMY22} since it is not publicly available.} Specifically, we run the measurement tool developed by Gotze et al.~\cite{GotzeMISL22} on all three datasets to collect the relevant data, which we then process to assess tracker prevalence and popularity.

The results show that the share of governmental websites with at least one third-party cookie set by a known tracker is similar across datasets: 10\% for the gpt-oss filtered dataset, 8.3\% for Singanamalla et al., and 8.9\% for Gotze et al. This suggests that conclusions drawn using our LLM-filtered version of Tranco are reliable, closely matching those obtained from two independent, curated datasets. 
%The largest observed difference is only 1.7\%, between the gpt-oss filtered dataset and the Singanamalla et al. dataset. While some variation is expected due to differences in the specific websites included, the overall trends are preserved, indicating that all three datasets are representative and support consistent privacy inferences.
%\SC{Forse le ultime due frasi si possono togliere / accorciare per recuperare spazio.}

Since the tracking ecosystem has been changing over the last few years, with trackers relying less on third-party cookies due to improved browser privacy protections~\cite{MunirSIEST23}, we performed a second experiment to better appreciate other privacy trends measurable in our dataset. Concretely, we extracted all the script tags available in the body of the HTML documents accessed in our measurement and used the Disconnect list to identify the most prevalent (first-party) trackers for each dataset. Our analysis of the top ten most prevalent trackers shows strong agreement across datasets, with the top six trackers identical in all three datasets and the top four also appearing in the same relative order of prevalence. Trackers at positions eight and nine are likewise consistent across datasets, while differences are observed only at positions seven and ten. Detailed results are reported in Table~\ref{tab:popular_script_trackers} in Appendix ~\ref{app:trackers_analysis}. Overall, these findings further confirm that the gpt-oss filtered dataset is representative, as it enables research inferences consistent with those derived from independent, curated datasets from the literature.

%As trackers increasingly rely less on third-party cookies due to improved browser privacy protections~\cite{MunirSIEST23}, we ran a second experiment to examine other privacy trends. We extracted all script tags from the HTML documents and used the Disconnect list to identify the most prevalent first-party trackers in each dataset. Table~\ref{tab:popular_script_trackers} lists the top trackers, with bold entries indicating identical ranks across datasets and italics showing consistent top-ten presence in different positions. Our analysis shows strong agreement: the top six trackers are identical, with the top four in the same order; positions eight and nine are also consistent, with minor differences at seven and ten. These results confirm that the gpt-oss filtered dataset is representative and supports research inferences consistent with independent curated datasets.

%\SC{Forse direi che il nostro è rappresentativo perché si allinea a dataset già proposti in letteratura. Tre dataset potrebbero essere allineati e non essere comunque rappresentativi.}
%\SC{Sezione 6 dovrebbe anche discutere le performance, che sono importanti per large-scale measurements. Teniamo traccia di quanto ci ha messo a classificare 100k siti per i vari task.}
%\SB{Da spiegare meglio come mai il nostro grafico è diverso rispetto a quello del paper originale (da controllare se sia così). Da chiarire se abbiamo rieseguito il crawl, in teoria è per quello che i grafici son diversi, ma non sappiamo il motivo esatto...}
%\SB{I commenti dei revisori di www: You are not testing the statistical significance of the result difference, How can you compare with [43] when that work is about HTTPS adoption? I have not found anything in that work about third-party tracking (or use of Disconnect).}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.45]{plots/paper_results_with_third_party_cookies_and_trackers_comparison_final.png}
%     \caption{\writtenbySB{Percentage of websites per country with third-party cookies set by a known tracker, across the three datasets.}}
%     \label{fig:gov_third_party}
% \end{figure}

\subsection{Privacy of Pornographic Websites}
\label{sec:porn_privacy_analysis}
%\SC{Questa sezione è un wall of text ed andrebbe ristrutturata in subsubsections. Nella prima penso che due fossero sufficienti e le ho messe io, qui da capire meglio.}

%Similar to our study on governmental websites, in this second study we construct a dataset of pornographic websites and analyze the privacy risks associated with visiting them. In particular, we investigate whether using an LLM-filtered version of the Tranco list can yield research inferences comparable to those obtained from datasets in previous work~\cite{VallinaFGVA19}, which require carefully curated, ad-hoc heuristics to build. Since the dataset from the prior study by Vallina et al.~\cite{VallinaFGVA19} is not publicly available, we first replicate their methodology to reconstruct it. We then build our gpt-oss filtered dataset, evaluate its quality, compare it to a keyword-based heuristic approach, and finally compare the privacy inferences derived from the reconstructed dataset and the gpt-oss filtered dataset.

%\subsubsection{Dataset Construction.}

%Previous work~\cite{VallinaFGVA19} on measuring privacy risks in pornographic websites constructed their dataset through three heuristics: $(i)$ filtered the Alexa Top list to retain only URLs containing keywords strongly indicative of pornographic content (e.g., ``porn'' and ``sex''), $(ii)$ scraped websites specialized in aggregating, recommending, and classifying pornographic content, and $(iii)$ included domains categorized as ``Adult'' by Alexa’s website classification service. Since their dataset is not publicly available, we reconstructed it by replicating their methodology as closely as possible. Because Alexa has been discontinued, we replaced it with the Tranco list, selecting the top 50k and bottom 50k domains to cover websites with different popularity. We replicated the original approach by filtering the selected Tranco domains using the same set of keywords reported in the paper for step $(i)$ and supplemented the resulting list with domains obtained by scraping the same three websites used in the original study~\cite{only4adults,mypornbible,toppornsites} for step $(ii)$. Unfortunately, unlike Alexa, Tranco does not provide website categories. Given this difference, we omit step $(iii)$ in our dataset reconstruction. Considering that the original methodology extracted just 22 websites using Alexa's categorization, we consider this change acceptable. The final reconstructed dataset contains 1,045 websites, of which 225 originate from the scraping phase. 
%To assess its quality, we randomly sampled 50 websites and manually inspected them. Of these, 48 (96\%) were indeed pornographic, indicating that the reconstructed dataset has a high level of precision.
%\SC{Un paio di commenti. Ridurrei l'elenco delle parole chiave, tenendo solo porn e sex, per evitare qualsiasi tipo di potenziale rottura di balle dai revisori. C'è un un punto di disconnessione perché Alexa ha una categoria Adult, mentre Tranco non ha le categorie, quindi la metodologia non generalizza direttamente. Da chiarire. Altra piccola nota: come nell'esperimento precedente sembra che le euristiche base diano accuratezza più alta. Un punto qui forse non detto abbastanza è che sono molto limitate di fatto, forse lo facevamo meglio per governmental perché li vedevamo che il dataset dei gov era quasi un subset del nostro.}

%We then used gpt-oss to build a dataset of pornographic websites to use in our measurement. In particular, we fed the same list of websites from Tranco to gpt-oss and asked it to classify each domain as pornographic or non-pornographic based solely on the URL. This first filtering step identified 8,949 domains as pornographic. To improve the quality of the dataset and reduce the number of false positives, we reclassified these domains by granting gpt-oss live access to the corresponding websites, as in our previous study. After this refinement, the final dataset consists of 2,936 websites. 
%\revision{In total, the two-phase filtering process took approximately 9 days and 19 hours, 9 days and 6 hours for the first phase and 13 hours for the second phase (details in Appendix~\ref{app:scalability}).} 
%To assess the quality of the dataset, we manually inspected 50 randomly sampled websites. Of these, 45 (90\%) were indeed pornographic, suggesting that the quality of the final dataset is high.
%\SC{Andrebbe motivato meglio perchè qui facciamo questo secondo passaggio e nel primo caso no. Forse perchè gov facevamo bene senza RAG, mentre questo è un problema di categorizzazione per cui la RAG sembrava importante? Forse non è neppure molto chiaro che non abbiamo usato la RAG nell'esperimento precedente, da chiarire.}

%To evaluate the effectiveness of gpt-oss filtering over Tranco, we compare the LLM-filtered dataset against the baseline dataset obtained by filtering the same Tranco domains with the set of keywords from Vallina et al.~\cite{VallinaFGVA19}.\footnote{For this comparison, we exclude from the baseline the websites obtained via scraping, as these domains are not present in Tranco and would inevitably be missed by gpt-oss.} The considered baseline includes 887 domains. Of these, 761 domains are present in both datasets, representing 86\% of the baseline. The baseline contains 126 domains that are not present in the gpt-oss dataset, while the gpt-oss filtered dataset includes an additional 2,175 domains not found in the baseline. Considering that the estimated precision of the two datasets is very high and that the baseline is, essentially, a subset of the gpt-oss filtered dataset, these results suggest that gpt-oss is able to construct a substantially larger and more comprehensive dataset while maintaining high accuracy (90\%), thereby correctly capturing many more pornographic domains.
%Moreover, unlike ad-hoc keyword-based heuristics, the gpt-oss approach is general and can be applied beyond the specific case of pornographic websites.
%\SC{Un po' debole il discorso sulla generalità, lo abbiamo già spiegato e va molto al di là di questo caso di studio specifico. In questo punto è più importante dire che siamo in qualche senso meglio nel caso specifico. Questa nota è anche correlata alla mia nota precedente, forse la presentazione va resa un po' più coesa perché il calo di accuracy da 96 a 90 è rilevante, quindi va chiarito subito che in realtà abbiamo un vantaggio sui numeri.}

%We then compare the gpt-oss filtered dataset with the one reconstructed using the heuristics of Vallina et al. by restricting the comparison to domains appearing in the Tranco top 50k and bottom 50k lists to ensure fairness. \SC{Qui non ci vedo fairness, ma una restrizione arbitraria. Magari il filtraggio può spiegare certi fenomeni che non ti aspetti, ma un dataset di riferimento ha valore solo se lo usi così com'è. Forse è solo un problema di wording? Nel senso che qui fai una prima analisi superficiale per capire l'overlap, ma nel seguito usi il dataset as is? Poco chiaro comunque.} Under this constraint, the reconstructed dataset is reduced to 

%\subsubsection{Web Measurement.}

Similarly to our governmental website study, our second study focuses on the privacy risks associated with visiting pornographic websites. Specifically, we evaluate whether our methodology can construct a dataset that yields research inferences comparable to those obtained in prior work~\cite{VallinaFGVA19}, which relied on carefully curated ad-hoc heuristics for dataset construction. Since the dataset used by Vallina et al.~\cite{VallinaFGVA19} is not publicly available, we first replicate their methodology to reconstruct it (details in Appendix~\ref{app:measurement_dataset_construction}), resulting in a dataset of 1,045 pornographic websites. To assess the representativeness of our gpt-oss filtered dataset and determine whether it supports meaningful research inferences, we repeat the privacy analysis described in Section~\ref{sec:gov_privacy_analysis}. In particular, we measure the prevalence and popularity of trackers embedded in third-party cookies and scripts, and compare the conclusions obtained from the gpt-oss dataset with those derived from the reconstructed dataset obtained by replicating Vallina et al.’s methodology. We conduct this analysis by running the tool introduced by Gotze et al.~\cite{GotzeMISL22} on both datasets and evaluating tracker prevalence and popularity according to the Disconnect list~\cite{disconnect_tracking_protection}. Overall, 34.8\% of websites in the reconstructed dataset set at least one third-party tracking cookie, compared to 23\% in the gpt-oss filtered dataset. At first glance, this difference might suggest that the two datasets lead to different privacy inferences.

%\SC{La tabella in appendice andrebbe assolutamente messa qui nel body, perchè il testo non è leggibile senza quella a supporto. Può essere che sia un problema dovuto alla difficile comprensibilità del paragrafo dopo, con una migliore ristrutturazione forse la tabella non serve più. Vedi commento dopo.}

%However, a more fine-grained analysis reveals a consistent trend across both datasets when splitting domains by popularity (Tranco top 50k vs. bottom 50k). In the reconstructed dataset, 26.1\% of websites in the Tranco top 50k set third-party tracking cookies, whereas this percentage increases to 38.7\% among those in the Tranco bottom 50k. A similar pattern emerges in the gpt-oss dataset: 19.5\% of domains in the Tranco top 50k set third-party tracking cookies, compared to 26.5\% in the bottom 50k. These results indicate that, despite differences in absolute prevalence, both datasets consistently capture the same underlying trend: more popular websites tend to exhibit a lower prevalence of third-party tracking cookies than less popular ones.
%\SC{Messa così, it appears out of the blue. Nessuno ha detto che questo è il trend che ti aspetti e che vuoi catturare. C'è una citazione per supportarlo? Altrimenti sembra veramente arbitrario. Inoltre mi sembra che siamo veramente dismissive nei confronti di un risultato che non ci piace. I numeri sono diversi, non possiamo semplicemente guardare altri numeri e fare finta che la differenza non sia un problema. Forse una soluzione è semplicemente togliere l'ultimo confronto ed integrare subito la parte qui sotto, che mi sembra più convincente, cioè ci sono delle differenze, ma anche delle similarità che riusciamo a misurare.}

To gain a better understanding of the observed differences, we analyzed the number of distinct third-party cookie trackers in the two datasets. The gpt-oss filtered dataset contains 126 distinct trackers, while the reconstructed dataset contains 50, with an intersection of 49 trackers. This corresponds to 98\% of the smaller set, indicating a strong alignment between the datasets. We further compared the third-party cookie trackers in the two datasets after filtering by website popularity (Tranco top 50k vs. bottom 50k). In the gpt-oss filtered dataset, we found 90 distinct trackers among the most popular websites and 79 among the least popular ones, while the reconstructed dataset has 32 and 38, respectively. Among the most popular websites, 30 trackers are shared between the datasets (93.8\% of the size of the smaller set), while among the least popular websites, the intersection is 34 trackers (89.5\% of the size of the smaller set). These results demonstrate a strong consistency between the datasets in capturing the set of trackers, even across popularity groups.

Additionally, when comparing the trackers in the most and least popular websites within each dataset, the intersection is 43 trackers (54.4\% of the size of the smaller set) in the gpt-oss filtered dataset and 20 trackers (62.5\% of the size of the smaller set) in the reconstructed dataset. This indicates that while popular and less popular websites embed substantially different trackers, both datasets consistently reflect this distinction. In other words, the two datasets lead to the same conclusion regarding how third-party cookie trackers vary with website popularity. Moreover, this trend aligns with the findings of Vallina et al.~\cite{VallinaFGVA19}, who reported very limited overlap of third-party domains across the popularity intervals they analyzed. In Table~\ref{tab:distinct-cookie-trackers-porno} (Appendix~\ref{app:trackers_analysis}) we summarize the statistics about third-party cookie trackers.
%Detailed results are presented in Table~\ref{tab:distinct-cookie-trackers-porno} (Appendix~\ref{app:trackers_analysis}).

%\SC{Qui richiediamo troppo sforzo cognitivo al lettore, perchè gli chiediamo di tenere in mente quattro numeri e concludiamo con due messaggi. A mio avviso bisogna prima di tutto confrontare gpt-oss vs Vallina e dire che i tracker sono in larga parte gli stessi, che è un finding fondamentale. Solo dopo andiamo a rompere i due dataset su popolarità ed osserviamo lo stesso fenomeno che avevano visto loro e quindi rinforziamo il messaggio.}
%To better understand tracker prevalence, we analyzed the number of distinct third-party cookie trackers in the two datasets, filtering websites by popularity (Tranco top 50k vs. bottom 50k; Table~\ref{tab:distinct-cookie-trackers-porno}). In the gpt-oss dataset, we found 90 trackers among the most popular sites and 79 among the least, with 43 (54.4% of the smaller set) in common. In the reconstructed dataset, there were 32 and 38 trackers for the most and least popular sites, respectively, with 20 (62.5%) shared. Comparing datasets, the intersection among the most popular sites is 30 trackers (93.8%) and 34 (89.5%) for the least popular. These results show that while popular and less popular websites embed different trackers, both datasets consistently capture this distinction. This trend aligns with Vallina et al.~\cite{VallinaFGVA19}, who observed limited overlap of third-party domains across popularity intervals.
%\SC{Questa parte è difficile da leggere senza una tabellina a supporto riguardo alla dimensione dei vari set / overlap. A livello di scrittura, cambierei ``maximum size of the intersection'' con ``size of the smaller set'', che è meno difficile da visualizzare (maximum è qualcosa che può crescere o calare, l'altro è un valore fisso).}
%\LC{Imho Tab.8 può andare in appendice: son d'accordo che rifarsi solo ai numeri nel testo non rende semplicissimo seguire, ma è anche vero che nel testo hai tutte le info che sono anche riportate nella tabella, a differenza di altre tabelle di questa sezione o di quella precedente che mostrano dati non riportati precisamente nel testo, ma a supporto di osservazioni. La lascerei, quindi, di supporto, ma se dobbiamo guadagnare spazio la muoverei in appendice.}

Finally, we analyzed the top ten most popular first-party trackers in the two datasets, using the same methodology adopted in the study on governmental websites (Section~\ref{sec:gov_privacy_analysis}). Our results show that both datasets support very similar conclusions: eight out of the top ten trackers are shared between them, i.e., the two datasets allow to capture almost the same popular trackers. Although the exact ranking positions are not preserved, the top two trackers are identical in both datasets. This strong overlap underscores a substantial alignment between the gpt-oss filtered dataset and the reconstructed dataset from the literature. It confirms the representativeness of the gpt-oss filtered dataset, as it leads to the same privacy-related inferences, i.e., the set of most popular trackers is preserved. Detailed results are reported in Table~\ref{tab:popular_script_trackers_porno} in Appendix ~\ref{app:trackers_analysis}.
%\SC{Forse relative popularity? Immagino che i numeri assoluti siano diversi.}
%\SC{Non ci sono entry in bold, quindi non serve scriverlo. La spiegazione è un po' involved (all trackers except two coincide in positions three through six). A livello di scrittura, manca un po' una storia: questo è un dato, un fatto, ma non stai spiegando veramente perché è un fatto importante e interessante. Qui l'inferenza principale che preservi sono l'insieme dei tracker più popolari.}


==> scratch.tex <==
\subsection{Classification Times}
\SC{All'inizio della sezione parlavamo di Scalability, perché ora usiamo Classification Times? Qual è più accurato? Mi sembra che stiamo mixando le due cose. Forse vogliamo analizzare in questa sezione i tempi puri e poi studiare nella prossima la scalabilità a livello di measurement, anche perché la metodologia a due fasi nasce esattamente per garantire la scalabilità.}
\label{sec:scalability}

%\SC{Qui dobbiamo fare vedere il trade-off fra classificare senza accesso al sito e con accesso al sito. Realisticamente implicato dalla scalability analysis.}

Having established that gpt-oss is accurate enough for large-scale web measurements, we now turn to the second experimental axis, i.e., the scalability of LLM-based classification, i.e., whether predictions are provided within time budgets compatible with building targeted datasets. %of thousands of websites.
\SC{Doppio i.e. da evitare. Non sono sicuro che la spiegazione sia accurata: building targeted datasets o fare targeted measurements? Gli esperimenti dopo suggerirebbero la seconda.}
 
\subsubsection{Setup.}
We measure per-website classification times for gpt-oss, our best-performing model, on the top 1k Tranco websites under the two previously used configurations, i.e., with and without live access (Section~\ref{sec:setup}). 
\SC{Perchè su Tranco? Vista la sezione, sembrerebbe naturale fare quest'analisi sui dataset che abbiamo usato per valutare la classification performance. A livello di valutazione: un solo modello su un solo task sembra poco rispetto alla valutazione precedente (più modelli su più task). Magari llama è molto più veloce di gpt-oss e per certi task va bene comunque. Per completezza mi sembrerebbe utile avere una valutazione comprensiva.}
We focus the analysis on the governmental website detection; the same considerations and conclusions apply to the other classification tasks. For each website and configuration, we measure the end-to-end classification time, i.e., the interval between submitting the prompt and receiving the final output. This includes both model inference and, when applicable, the time the LLM spends visiting and processing the website. To obtain statistically robust estimates, we repeat each measurement five times and report the per-website average. Finally, to reflect realistic deployment constraints, we cap each classification at a 30-second timeout, since targeted dataset construction can involve classifying 100k websites or more and excessive per-website times would make measurements impractical.

%As the reference baseline, we also measure the time required to visit each website, since this operation represents an unavoidable cost for any targeted measurement pipeline, as well as for human-based and some heuristic-based website classification approaches (Section~\ref{sec:benchmark}). We refer the reader to Appendix~\ref{app:scalability_setup} for the full experimental details, including the size of the website sample, the timeout, and the number of repetitions.

%\SB{Non so se qui o sotto, però chiarirei un po' meglio forse il fatto che per i targeted web measurement senza un llm devi visitare tutti i siti per poterli classificare, però non ti serve visitarli tutti per fare il measurement a differenza dei web measurement non targeted. Quindi si può sfruttare il vantaggio dell'LLM che non visita tutti i siti. Quello che intendo è di chiarire la differenza tra classificazione e measurement, e cosa serve che visiti in uno e nell'altro e quindi come consideri i tempi.}
%\SC{Secondo me qui dovremmo già chiarire che facciamo tante run per rappresentatività statistica, altrimenti sembra lazy: un modello ed un task, invece di N modelli e tre task. Andrebbe chiarito meglio il quadro. Concordo con Simone che il riferimento ai tempi di navigazione potrebbe essere più chiaro. Forse si può evitare di discuterlo qui e prenderlo semplicemente come baseline sotto.}

\subsubsection{Results.}
%\LC{Da asciugare e aggiungere qualche riferimento alla sezione precedente}
Figure~\ref{fig:scalability_distribution} shows the distribution of per-website classification times for the governmental classification task across the two configurations. Blue denotes the configuration without live access, orange the one with access enabled.
 %, alongside the time required to visit the websites. 
 
Overall, the results indicate that LLM-based classification scales well. Across the configurations, the median classification time stays below 2 seconds, and even with live access enabled the mean remains below 4 seconds. This is fast enough to support filtering on lists of websites of reasonable size. For example, classifying 100k websites with access enabled would require around 4 and half days on average, which is in line with the duration of large-scale web measurement studies in the literature~\cite{SinganamallaJAK20,SamarasingheAMY22,ZengWGKR21}.
 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/time_governmental_vs_visit.pdf}
    \caption{Website classification time distributions with live website access (orange) and without access (blue) for the governmental classification task, along with website visit times only. For readability, the distributions are truncated around 11 seconds.}%, omitting extreme outliers.}
    \label{fig:scalability_distribution}
\end{figure}
%Each box represents the interquartile range (25th--75th percentiles), and dashed ticks indicate the mean. Outliers beyond the whiskers are plotted individually.
 
Enabling website access, however, increases variability and average classification time, yielding heavier-tailed distributions (longer whiskers in the orange boxplot). The mean classification time rises from 2.6 to 3.8 seconds, due to the overhead of retrieving website content when the LLM decides to access it. The one-sided Wilcoxon signed-rank test, a paired non-parametric test evaluating whether enabling live access increases classification time relative to the no-access configuration, confirms that this increase is statistically significant ($p = 2.21\times10^{-23}$). The impact of this increase depends on the size of the list to filter. For a moderate size of the list of websites to filter, e.g. 100k candidates, enabling live access adds only about 1 day and 9 hours of total classification time on average (approximately 3 days without access vs.\ 4 days and 9 hours with access), so classification with live access remains a viable option, although less efficient. However, for larger lists the gap becomes substantial: filtering the Tranco top 1M with live access requires approximately 14 days more than without it on average (30 days and 2 hours without access vs.\ 43 days and 23 hours with access), making the no-access configuration the preferable choice when classification has to scale to large website lists.

%\SB{mettiamo i totali tra parentesi? (oltre ai delta)}

%Estimates:
%3 days without website access on average for 100k websites
%4 days and 9 hours with website access on average for 100k websites

%1M without access: 30 days and 2 hours, 722.222 hours
%1M with access: 43 days and 23 hours, 1055,555 hours

%Despite this overhead, classification with live access remains significantly faster than pure website visits ($p = 2.59\times10^{-54}$, same test), because the LLM can skip the visit in some cases, whereas manual or heuristic classification pipelines must always load the page.
\SC{Mi sembrerebbe di poter dire che tutta la parte qui sotto è funzionale alla metodologia a due fasi. Ci sono vari punti interessanti qui, che rischiano di essere ignorati da un lettore superficiale che decide banalmente di saltare la parte sui tempi di classificazione. Penso che starebbe meglio nella Sezione 6, facendo opportuni aggiustamenti alle due parti, oppure in una take-away subsection. Stiamo mixando tempi di classificazione con scalabilità, due concetti collegati ma distinti.}
To contextualize these classification times, we adopt as a baseline the time required to visit each website without invoking the LLM, measured under the same setup and shown in the rightmost green boxplot of Figure~\ref{fig:scalability_distribution}. We note that the classification times are consistently lower than this baseline (6.3 seconds mean) and the same Wilcoxon signed-rank test confirms the difference is statistically significant even with live access enabled ($p = 2.59\times10^{-54}$). This occurs because the LLM does not always visit the website before labeling it: as discussed in Section~\ref{sec:setup}, the pipeline allows the model to skip visits when its existing knowledge is sufficient. This is a key advantage of LLM-based classification in the context of \emph{targeted} web measurements. Unlike non-targeted measurements, in which every website of an input list (such as Tranco) is visited, targeted measurements proceed by first \emph{filtering} every candidate website to identify the subset of interest, and by \emph{measuring} only on that retained subset. Ideally, the visit cost should be paid only for the websites belonging to the target class. However, manual classification and content-based heuristic classifiers must visit every candidate during filtering, regardless of the class. On the other hand, the LLM-based pipeline allows for reducing the cost of the filtering process by skipping some visits.

%More importantly, classification times are consistently lower than the website visit times reported on the right of the figure (6.3 seconds mean) and the same Wilcoxon signed-rank test confirms that this difference is statistically significant even when live access is enabled ($p = 2.59\times10^{-54}$). This is the case even when live access is enabled, because the LLM does not necessarily visit the website before returning a label: as discussed in Section~\ref{sec:setup}, the classification pipeline lets the model skip the visit whenever the LLM considers existing knowledge of the target domain to be sufficient. This is the key advantage of LLM-based classification over manual or heuristic-based alternatives: these approaches typically need to access each website and therefore must load every page to be classified, while with an LLM this cost can be avoided in some cases. 

%since the LLM may decide to skip it for classifying and relying on its knowledge to classify a website.

%The same per-page visit cost is, however, already paid by any web measurement pipeline when collecting its actual measurements: a heuristic-based pipeline thus pays the visit cost twice per website, once for classification and once for the measurement itself. 
% With an LLM, this cost can be avoided, since the LLM may decide to skip it for classifying and relying on its knowledge to classify a website.
%, in many cases, skipped altogether. The fact that the LLM's classification time is, on average, smaller than a single website visit confirms this saving empirically and shows that LLM-based classification is best understood not as an additional cost on top of classic measurement pipelines, but as a way to reduce the visit overhead practitioners are already paying.

To sum up, the results show that $(i)$ LLMs enable scalable construction of targeted datasets for web measurements; $(ii)$ a clear trade-off emerges, enabling live access improves accuracy (Section~\ref{sec:classification-performance}) but increases variability and average classification time, with the gap between the two configurations growing substantially for large input lists; and $(iii)$ LLM-based classification is cheaper than a standard website visit, making it a more effective and efficient alternative to manual or heuristic-based approaches.

%The first two findings also motivate the two-stage filtering strategy adopted in our privacy studies (Sections~\ref{sec:gov_privacy_analysis} and~\ref{sec:porn_privacy_analysis}): we first run gpt-oss without website access to efficiently filter a large list of websites, then perform a second, more expensive classification with access enabled on the filtered subset to confirm labels. This approach balances scalability and accuracy and is our recommended recipe for LLM-based web measurement pipelines.}
